A Liquid Scintillation Detector for Radioassay of Gadolinium-Loaded Liquid Scintillator for the LZ Outer Detector

We report on the design and performance of the LUX-ZEPLIN (LZ) "Screener", a small liquid scintillator detector consisting of $\approx 23$ kg of LAB-based gadolinium-loaded liquid scintillator (GdLS) to be used in the LZ Outer Detector. The Outer Detector will be filled with 17.3 tonnes of GdLS and will surround the central liquid xenon time projection chamber of LZ. Its primary function will be to veto neutron single-scatter events in the liquid xenon which could mimic a WIMP dark matter signal. To meet the requirements for the Outer Detector, the radioimpurity levels in the GdLS must be kept below $\lesssim0.07$ mBq/kg. This background level corresponds to a rate of $\approx50$ Hz above an energy threshold of 100 keV. The Screener was operated in the ultra-low-background environment of the former LUX water shield in the Davis Laboratory at the Sanford Underground Research Facility for radioassay of the GdLS. Careful selection of detector materials and use of ultra-low-background PMTs allows the measurement of a variety of radioimpurities. The $^{14}\textrm{C}$/$^{12}\textrm{C}$ ratio in the scintillator is measured to be $(2.83\pm0.06\textrm{(stat.)}\pm0.01\textrm{(sys.)}) \times 10^{-17}$. Use of pulse shape discrimination allows the concentration of isotopes throughout the $^{238}\textrm{U}$, $^{235}\textrm{U}$, and $^{232}\textrm{Th}$ chains to be measured by fitting the collected spectra from $\alpha$ and $\beta$ events. We find that equilibrium is broken in the $^{238}\textrm{U}$ and $^{232}\textrm{Th}$ chains and that a significant portion of the contamination in the GdLS results from decays in the $^{227}\textrm{Ac}$ subchain of the $^{235}\textrm{U}$ series. Predictions for the singles rate in the Outer Detector are presented. The rate from radioimpurities above 100 keV in the GdLS is estimated to be $97.9\pm6.4$ Hz, with $65.5\pm1.9$ Hz resulting from $\alpha$-decays.

==> LZPaperSupport/LZsym.tex <==
%%%%%   Symbols for use in LZ
%%%%%
%%%%%   Revised from BaBar/SuperB/accelerator to LZ  08/17/2015  H. Nelson
%%%%%

\RequirePackage{xspace}

\RequirePackage{hyperref}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\mathrm{t}}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\mathrm{t}}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\mathrm{ES}}$}\xspace}
\def\mec        {\mbox{$m_{\mathrm{EC}}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\keVee}{\si{\keV\ee}}
%\newcommand{\keVnr}{\si{\keV\nr}}
%\newcommand{\keVvis}{\si{\keV\vis}}
\DeclareRobustCommand{\Pga}{\HepParticle{\alpha}{}{}\xspace} % alpha
\DeclareRobustCommand{\Pgb}{\HepParticle{\beta}{}{}\xspace} % beta
\DeclareRobustCommand{\Pgd}{\HepParticle{\delta}{}{}\xspace} % delta
\DeclareRobustCommand{\Pgbm}{\HepParticle{\beta}{}{-}\xspace} % negative beta
\DeclareRobustCommand{\Pgbp}{\HepParticle{\beta}{}{+}\xspace} % positive beta
\DeclareRobustCommand{\Pd}{\HepParticle{d}{}{}\xspace} % deuteron
\DeclareRobustCommand{\Pad}{\HepAntiParticle{d}{}{}\xspace} % anti-deuteron
\DeclareRobustCommand{\Pt}{\HepParticle{t}{}{}\xspace} % triton
\DeclareRobustCommand{\Pad}{\HepAntiParticle{t}{}{}\xspace} % anti-triton
%\newcommand{\perkkd}{\si{\per\keV\per\kg\per\day}} % /keV/kg/day
%\newcommand{\perkgd}{\si{\per\keV\per\day}} % /kg/day
%\newcommand{\perktd}{\si{\per\keV\per\tonne\per\day}} % /keV/tonne/day
%\newcommand{\pertd}{\si{\per\tonne\per\day}} % /tonne/day
%\newcommand{\perkty}{\si{\per\keV\per\tonne\per\year}} % /keV/tonne/year
%\newcommand{\perty}{\si{\per\tonne\per\year}} % /tonne/year

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\,\mathrfm{in}}\xspace} % \in is taken
\def\ft   {\ensuremath{\,\mathrfm{ft}}\xspace}
\def\km   {\ensuremath{{\,\mathrm{km}}}\xspace}
\def\m    {\ensuremath{{\,\mathrm{m}}}\xspace}
\def\msquare {\ensuremath{{\,\mathrm{m}}^2}\xspace}
\def\cm   {\ensuremath{{\,\mathrm{cm}}}\xspace}
\def\cma  {\ensuremath{{\,\mathrm{cm}}^2}\xspace}
\def\cubicm   {\ensuremath{{\,\mathrm{m}}^3}\xspace}
\def\mm   {\ensuremath{{\,\mathrm{mm}}}\xspace}
\def\mma  {\ensuremath{{\,\mathrm{mm}}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\mathrm{m}}}\xspace}%% mu meter
\def\muma {\ensuremath{{\,\mu\mathrm{m}}^2}\xspace}
\def\nm   {\ensuremath{{\,\mathrm{nm}}}\xspace}
\def\fm   {\ensuremath{{\,\mathrm{fm}}}\xspace}
\def\nm   {\ensuremath{{\,\mathrm{nm}}}\xspace}   %% nanometer
%
% integrated cross section, exposure
\def\barn{\ensuremath{{\,\mathrm{b}}}\xspace}
\def\barnhyph{\ensuremath{{\mathrm{-b}}}\xspace}
\def\mbarn{\ensuremath{{\,\mathrm{mb}}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb{\ensuremath{{\,\mathrm{nb}}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\,\mathrm{pb}}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ab   {\ensuremath{\mbox{\,ab}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}
\def\designlumi {\ensuremath{10^{36}\cms}\xspace}
\def\lumi {\cms\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\,\mus}\xspace}
\def\ns   {\ensuremath{\,\mathrm{ns}}\xspace}
\def\ps   {\ensuremath{\,\mathrm{ps}}\xspace}
\def\fs   {\ensuremath{\,\mathrm{fs}}\xspace}

%Mass
\def\gm   {\ensuremath{\,\mathrm{g}}\xspace}
\def\kg   {\ensuremath{\,\mathrfm{kg}}\xspace}
\def\ton  {\ensuremath{{\,\mathrm{t}}}\xspace}

\def\gmps {\ensuremath{\,\mathrm{g/s}}\xspace} 


%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{{\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\,\mathrm{ms}}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu\mathrm{s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\,\mathrm{ns}}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\,\mathrm{ps}}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\eg{\ensuremath\mathrm{e.g.}}
\def\ie{\ensuremath\mathrm{i.e.}}

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\pct {\ensuremath{{\,\mathrm{\%}}}\xspace}

\def\cms         {\ensuremath{{\,\mathrm{cm}}^{-2} {s}^{-1}}\xspace}

\def\muF  {\ensuremath{\,\mu\mathrm{F}}\xspace}
\def\muH  {\ensuremath{\,\mu\mathrm{H}}\xspace}
\def\nF   {\ensuremath{\,\mathrm{nF}}\xspace}
\def\nH   {\ensuremath{\,\mathrm{nH}}\xspace}
\def\mic  {\ensuremath{\,\mu\mathrm{C}}\xspace}
\def\krad {\ensuremath{\,\mathrm{krad}}\xspace}
\def\cmc  {\ensuremath{{\,\mathrm{cm}}^3}\xspace}
\def\yr   {\ensuremath{\,\mathrm{yr}}\xspace}
\def\hr   {\ensuremath{\,\mathrm{hr}}\xspace}
\def\degc {\ensuremath{^\circ}{\mathrm{C}}\xspace}
\def\degk {\ensuremath {\,\mathrm{K}}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\,\mathrm{mrad}}\xspace}               %% milliradian
\def\rad{\ensuremath{\,\mathrm{rad}}\xspace}
\def\mradhyph{\ensuremath{\mathrm{-mr}}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}
\def\thlf  {\ensuremath{\mathrm{T}_{1/2}}\xspace}

%\renewcommand{\bar}[1]{\overline{#1}}

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing

\def\bit	{\ensuremath{{\,\text{bit}}}\xspace}
\def\kbit	{\ensuremath{{\,\text{kbit}}}\xspace}
\def\kbitps	{\ensuremath{{\,\text{kbit/s}}}\xspace}
\def\kbitsps	{\kbitps} % no more plural of units - deprecated
\def\kbps	{\kbitps} % for compatibility - deprecated
\def\kbsps	{\kbitsps} % for compatibility - deprecated

\def\kbyte      {\ensuremath{{\,\text{kByte}}}\xspace}
\def\kbytes	{\kbyte}
\def\kbyteps    {\ensuremath{{\,\text{kByte/s}}}\xspace}
\def\kbytesps	{\kbyteps}


\def\mbyte	{\ensuremath{{\,\text{MByte}}}\xspace}
\def\mbytes	{\mbyte}
\def\mbyteps	{\ensuremath{{\,\text{MByte/s}}}\xspace}
\def\mbytesps	{\mbyteps}

\def\mbit	{\ensuremath{{\,\text{Mbit}}}\xspace}
\def\mbits	{\mbit}
\def\mbitps	{\ensuremath{{\,\text{Mbit/s}}}\xspace}
\def\mbitsps	{\mbitps}
\def\mbps	{\mbitps} % for compatibility - deprecated
\def\mbsps	{\mbitsps} % for compatibility - deprecated

\def\gbit	{\ensuremath{{\,\text{Gbit}}}\xspace}
\def\gbits	{\gbit}
\def\gbitps	{\ensuremath{{\,\text{Gbit/s}}}\xspace}
\def\gbitsps	{\gbitps}
\def\gbps	{\gbitps} % for compatibility - deprecated
\def\gbsps	{\gbitsps} % for compatibility - deprecated


\def\gbyte	{\ensuremath{{\,\text{GByte}}}\xspace}
\def\gbytes	{\gbyte}
\def\gbyteps	{\ensuremath{{\,\text{GByte/s}}}\xspace}
\def\gbytesps	{\gbyteps}

\def\tbyte	{\ensuremath{{\,\text{TByte}}}\xspace}
\def\tbytes	{\tbyte}
\def\tbyteps	{\ensuremath{{\,\text{TByte/s}}}\xspace}
\def\tbytesps	{\tbyteps}
\def\tbyteph	{\ensuremath{{\,\text{TByte/h}}}\xspace}
\def\tbytesph   {\tbyteph}
\def\tbytepd	{\ensuremath{{\,\text{TByte/day}}}\xspace}
\def\tbytespd   {\tbytepd}

\def\pbyte	{\ensuremath{{\,\text{PByte}}}\xspace}
\def\pbytepy    {\ensuremath{{\,\text{PByte/yr}}}\xspace}

\def\tbpy       {\ensuremath{{\,\text{TByte/yr}}}\xspace}

\def\khs        {\ensuremath{{\,\text{kHS06}}}\xspace}
\def\mhs	{\ensuremath{{\,\text{MHS06}}}\xspace}

\def\tbpab	{\ensuremath{\tbyte/\invab}}
\def\khspab	{\ensuremath{\khs/\invab}}



\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{\ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

%
% Dark Matter
%
\newcommand{\vesc}{\ensuremath{v_{\text{esc}}}\xspace}
\newcommand{\MWIMP}{\ensuremath{M_{\text{WIMP}}}\xspace}
\newcommand{\Emin}{\ensuremath{E_{\text{min}}}\xspace}
\newcommand{\QBB}{\ensuremath{Q_{\!\Pgb\kern-0.1em\Pgb}}\xspace}

%
% Radioactive Isotopes
%
\newcommand{\IXenat}{\HepIsotope{Xe}{}{nat}\xspace}
\newcommand{\IXemes}{\HepIsotope{Xe}{}{m}\xspace}
\newcommand{\IXeotf}{\HepIsotope{Xe}{}{124}\xspace}
\newcommand{\IXeotF}{\HepIsotope{Xe}{}{125}\xspace}
\newcommand{\IXeots}{\HepIsotope{Xe}{}{126}\xspace}
\newcommand{\IXeotS}{\HepIsotope{Xe}{}{127}\xspace}
\newcommand{\IXeote}{\HepIsotope{Xe}{}{128}\xspace}
\newcommand{\IXeotn}{\HepIsotope{Xe}{}{129}\xspace}
\newcommand{\IXeotnm}{\HepIsotope{Xe}{}{129m}\xspace}
\newcommand{\IXeoTz}{\HepIsotope{Xe}{}{130}\xspace}
\newcommand{\IXeoTo}{\HepIsotope{Xe}{}{131}\xspace}
\newcommand{\IXeoTom}{\HepIsotope{Xe}{}{131m}\xspace}
\newcommand{\IXeoTt}{\HepIsotope{Xe}{}{132}\xspace}
\newcommand{\IXeoTT}{\HepIsotope{Xe}{}{133}\xspace}
\newcommand{\IXeoTf}{\HepIsotope{Xe}{}{134}\xspace}
\newcommand{\IXeoTF}{\HepIsotope{Xe}{}{135}\xspace}
\newcommand{\IXeoTs}{\HepIsotope{Xe}{}{136}\xspace}
\newcommand{\IKrnat}{\HepIsotope{Kr}{}{nat}\xspace}
\newcommand{\IKreF}{\HepIsotope{Kr}{}{85}\xspace}
\newcommand{\IKreTm}{\HepIsotope{Kr}{}{83m}\xspace}
\newcommand{\IKreT}{\HepIsotope{Kr}{}{83}\xspace}
\newcommand{\IRbeT}{\HepIsotope{Rb}{}{83}\xspace}
\newcommand{\IRntoe}{\HepIsotope{Rn}{}{218}\xspace}
\newcommand{\IRnton}{\HepIsotope{Rn}{}{219}\xspace}
\newcommand{\IRnttz}{\HepIsotope{Rn}{}{220}\xspace}
\newcommand{\IRnttt}{\HepIsotope{Rn}{}{222}\xspace}
\newcommand{\IHo}{\HepIsotope{H}{}{1}\xspace}
\newcommand{\IHt}{\HepIsotope{H}{}{2}\xspace}
\newcommand{\IHT}{\HepIsotope{H}{}{3}\xspace}
\newcommand{\IHeT}{\HepIsotope{He}{}{3}\xspace}
\newcommand{\IArTS}{\HepIsotope{Ar}{}{37}\xspace}
\newcommand{\IArTn}{\HepIsotope{Ar}{}{39}\xspace}
\newcommand{\IArnat}{\HepIsotope{Ar}{}{nat}\xspace}
\newcommand{\IUtTf}{\HepIsotope{U}{}{234}\xspace}
\newcommand{\IUtTF}{\HepIsotope{U}{}{235}\xspace}
\newcommand{\IUtTFE}{\HepIsotope{U}{}{235}$_{\mathrm{e}}$\xspace}
\newcommand{\IUtTFL}{\HepIsotope{U}{}{235}$_{\mathrm{l}}$\xspace}
\newcommand{\IUtTe}{\HepIsotope{U}{}{238}\xspace}
\newcommand{\IUtTeE}{\HepIsotope{U}{}{238}$_{\mathrm{e}}$\xspace}
\newcommand{\IUtTeM}{\HepIsotope{U}{}{238}$_{\mathrm{m}}$\xspace}
\newcommand{\IUtTeL}{\HepIsotope{U}{}{238}$_{\mathrm{l}}$\xspace}
\newcommand{\IUnat}{\HepIsotope{U}{}{nat}\xspace}
\newcommand{\IPatTo}{\HepIsotope{Pa}{}{231}\xspace}
\newcommand{\IPatTT}{\HepIsotope{Pa}{}{233}\xspace}
\newcommand{\IPatTf}{\HepIsotope{Pa}{}{234}\xspace}
\newcommand{\IPatTfm}{\HepIsotope{Pa}{}{234m}\xspace}
\newcommand{\IThttS}{\HepIsotope{Th}{}{227}\xspace}
\newcommand{\IThtte}{\HepIsotope{Th}{}{228}\xspace}
\newcommand{\IThtTz}{\HepIsotope{Th}{}{230}\xspace}
\newcommand{\IThtTo}{\HepIsotope{Th}{}{231}\xspace}
\newcommand{\IThtTt}{\HepIsotope{Th}{}{232}\xspace}
\newcommand{\IThtTtE}{\HepIsotope{Th}{}{232}$_{\mathrm{e}}$\xspace}
\newcommand{\IThtTtL}{\HepIsotope{Th}{}{232}$_{\mathrm{l}}$\xspace}
\newcommand{\IThtTf}{\HepIsotope{Th}{}{234}\xspace}
\newcommand{\IActtS}{\HepIsotope{Ac}{}{227}\xspace}
\newcommand{\IActte}{\HepIsotope{Ac}{}{228}\xspace}
\newcommand{\IRattT}{\HepIsotope{Ra}{}{223}\xspace}
\newcommand{\IRattf}{\HepIsotope{Ra}{}{224}\xspace}
\newcommand{\IRatts}{\HepIsotope{Ra}{}{226}\xspace}
\newcommand{\IRattS}{\HepIsotope{Ra}{}{227}\xspace}
\newcommand{\IRatte}{\HepIsotope{Ra}{}{228}\xspace}
\newcommand{\IFrttT}{\HepIsotope{Fr}{}{223}\xspace}
\newcommand{\IFrttf}{\HepIsotope{Fr}{}{224}\xspace}
\newcommand{\IAttoF}{\HepIsotope{At}{}{215}\xspace}
\newcommand{\IAttoe}{\HepIsotope{At}{}{218}\xspace}
\newcommand{\IAtton}{\HepIsotope{At}{}{219}\xspace}
\newcommand{\IPotoz}{\HepIsotope{Po}{}{210}\xspace}
\newcommand{\IPotoo}{\HepIsotope{Po}{}{211}\xspace}
\newcommand{\IPotot}{\HepIsotope{Po}{}{212}\xspace}
\newcommand{\IPotof}{\HepIsotope{Po}{}{214}\xspace}
\newcommand{\IPotoF}{\HepIsotope{Po}{}{215}\xspace}
\newcommand{\IPotos}{\HepIsotope{Po}{}{216}\xspace}
\newcommand{\IPotoe}{\HepIsotope{Po}{}{218}\xspace}
\newcommand{\IBitzF}{\HepIsotope{Bi}{}{205}\xspace}
\newcommand{\IBitzs}{\HepIsotope{Bi}{}{206}\xspace}
\newcommand{\IBitoz}{\HepIsotope{Bi}{}{210}\xspace}
\newcommand{\IBitoo}{\HepIsotope{Bi}{}{211}\xspace}
\newcommand{\IBitot}{\HepIsotope{Bi}{}{212}\xspace}
\newcommand{\IBitof}{\HepIsotope{Bi}{}{214}\xspace}
\newcommand{\IBitoF}{\HepIsotope{Bi}{}{215}\xspace}
\newcommand{\IPbtzs}{\HepIsotope{Pb}{}{206}\xspace}
\newcommand{\IPbtzS}{\HepIsotope{Pb}{}{207}\xspace}
\newcommand{\IPbtze}{\HepIsotope{Pb}{}{208}\xspace}
\newcommand{\IPbtoz}{\HepIsotope{Pb}{}{210}\xspace}
\newcommand{\IPbtot}{\HepIsotope{Pb}{}{212}\xspace}
\newcommand{\IPbtof}{\HepIsotope{Pb}{}{214}\xspace}
\newcommand{\ITltzs}{\HepIsotope{Tl}{}{206}\xspace}
\newcommand{\ITltzS}{\HepIsotope{Tl}{}{207}\xspace}
\newcommand{\ITltze}{\HepIsotope{Tl}{}{208}\xspace}
\newcommand{\ITltoz}{\HepIsotope{Tl}{}{210}\xspace}
\newcommand{\IHgtos}{\HepIsotope{Hg}{}{206}\xspace}
\newcommand{\IKfz}{\HepIsotope{K}{}{40}\xspace}
\newcommand{\IKnat}{\HepIsotope{K}{}{nat}\xspace}
\newcommand{\IScfs}{\HepIsotope{Sc}{}{46}\xspace}
\newcommand{\ICoFS}{\HepIsotope{Co}{}{57}\xspace}
\newcommand{\IKft}{\HepIsotope{K}{}{42}\xspace}
\newcommand{\IScffm}{\HepIsotope{Sc}{}{44,44m}\xspace}
\newcommand{\IScfS}{\HepIsotope{Sc}{}{47}\xspace}
\newcommand{\IScfe}{\HepIsotope{Sc}{}{48}\xspace}
\newcommand{\ICsoTS}{\HepIsotope{Cs}{}{137}\xspace}
\newcommand{\ICftFt}{\HepIsotope{Cf}{}{252}\xspace}
\newcommand{\ICosz}{\HepIsotope{Co}{}{60}\xspace}
\newcommand{\ICrFo}{\HepIsotope{Cr}{}{51}\xspace}
\newcommand{\IAmtfo}{\HepIsotope{Am}{}{241}\xspace}
\newcommand{\IYee}{\HepIsotope{Y}{}{88}\xspace}
\newcommand{\ICsoTs}{\HepIsotope{Cs}{}{136}\xspace}
\newcommand{\INatt}{\HepIsotope{Na}{}{22}\xspace}
\newcommand{\IBe}{\HepIsotope{B}{}{8}\xspace}
\newcommand{\IBeS}{\HepIsotope{Be}{}{7}\xspace}
\newcommand{\IBen}{\HepIsotope{Be}{}{9}\xspace}
\newcommand{\INoT}{\HepIsotope{N}{}{13}\xspace}
\newcommand{\INof}{\HepIsotope{N}{}{14}\xspace}
\newcommand{\IOoF}{\HepIsotope{O}{}{15}\xspace}
\newcommand{\IFoS}{\HepIsotope{F}{}{17}\xspace}
\newcommand{\Ipp}{\HepIsotope{p}{}{}\HepIsotope{p}{}{}\xspace}
\newcommand{\Ihep}{\HepIsotope{h}{}{}\HepIsotope{e}{}{}\HepIsotope{p}{}{}\xspace}
\newcommand{\Dnuenue}{\hbox{\Pgn\kern-0.3em\Pe\kern-0.3em$\to$\kern-0.1em\Pgn\kern-0.3em\Pe}\xspace}
\newcommand{\ISmofS}{\HepIsotope{Sm}{}{147}\xspace}
\newcommand{\ISmoFz}{\HepIsotope{Sm}{}{150}\xspace}
\newcommand{\ISmoFT}{\HepIsotope{Sm}{}{153}\xspace}
\newcommand{\IEuoFt}{\HepIsotope{Eu}{}{152}\xspace}
\newcommand{\IGd}{\HepIsotope{Gd}{}{}\xspace}
\newcommand{\IGdnat}{\HepIsotope{Gd}{}{nat}\xspace}
\newcommand{\IGdoFt}{\HepIsotope{Gd}{}{152}\xspace}
\newcommand{\IGdoFT}{\HepIsotope{Gd}{}{153}\xspace}
\newcommand{\IGdoFf}{\HepIsotope{Gd}{}{154}\xspace}
\newcommand{\IGdoFF}{\HepIsotope{Gd}{}{155}\xspace}
\newcommand{\IGdoFs}{\HepIsotope{Gd}{}{156}\xspace}
\newcommand{\IGdoFS}{\HepIsotope{Gd}{}{157}\xspace}
\newcommand{\IGdoFe}{\HepIsotope{Gd}{}{158}\xspace}
\newcommand{\IGdosz}{\HepIsotope{Gd}{}{160}\xspace}
\newcommand{\IGdcap}{\HepIsotope{Gd}{}{155,157}\xspace}
\newcommand{\ICot}{\HepIsotope{C}{}{12}\xspace}
\newcommand{\ICoT}{\HepIsotope{C}{}{13}\xspace}
\newcommand{\ICof}{\HepIsotope{C}{}{14}\xspace}
\newcommand{\ILaoTe}{\HepIsotope{La}{}{138}\xspace}
\newcommand{\INptTn}{\HepIsotope{Np}{}{239}\xspace}
\newcommand{\ICsoTf}{\HepIsotope{Cs}{}{134}\xspace}
\newcommand{\IIotF}{\HepIsotope{I}{}{125}\xspace}
\newcommand{\IIotS}{\HepIsotope{I}{}{127}\xspace}
\newcommand{\IIoTo}{\HepIsotope{I}{}{131}\xspace}
\newcommand{\ITeotom}{\HepIsotope{Te}{}{121m}\xspace}
\newcommand{\ITeotTm}{\HepIsotope{Te}{}{123m}\xspace}
\newcommand{\ILuoSs}{\HepIsotope{Lu}{}{176}\xspace}
%
%  Double Beta Decay
%
%\newcommand{\Pznbb}{\hbox{0\Pgn\kern-4pt\Pgb\kern-4pt\Pgb}}
\newcommand{\Dznbb}{\hbox{0\Pgn\kern-0.3em\Pgb\kern-0.35em\Pgb}\xspace}
\newcommand{\Dtnbb}{\hbox{2\Pgn\kern-0.3em\Pgb\kern-0.35em\Pgb}\xspace}

%
% Chemicals - intially single elements
%
\newcommand{\CNt}{\HepChemical{N}{2}{}\xspace}
\newcommand{\COt}{\HepChemical{O}{2}{}\xspace}
\newcommand{\COtM}{\HepChemical{O}{2}{-}\xspace}
\newcommand{\CHt}{\HepChemical{H}{2}{}\xspace}
\newcommand{\CHT}{\HepChemical{H}{3}{}\xspace}
\newcommand{\CHf}{\HepChemical{H}{4}{}\xspace}
\newcommand{\CHFi}{\HepChemical{H}{5}{}\xspace}
\newcommand{\CHs}{\HepChemical{H}{6}{}\xspace}
\newcommand{\CHoo}{\HepChemical{H}{11}{}}
\newcommand{\CHot}{\HepChemical{H}{12}{}\xspace}
\newcommand{\CHos}{\HepChemical{H}{16}{}\xspace}
\newcommand{\CHoS}{\HepChemical{H}{17}{}\xspace}
\newcommand{\CHoe}{\HepChemical{H}{18}{}\xspace}
\newcommand{\CHtt}{\HepChemical{H}{22}{}\xspace}
\newcommand{\CHGdLS}{\HepChemical{H}{28.128}{}\xspace}
\newcommand{\CHLAB}{\HepChemical{H}{28.28}{}\xspace}
\newcommand{\CHtN}{\HepChemical{H}{2n}{}\xspace}
\newcommand{\CCs}{\HepChemical{C}{6}{}\xspace}
\newcommand{\CCn}{\HepChemical{C}{9}{}\xspace}
\newcommand{\CCoF}{\HepChemical{C}{15}{}\xspace}
\newcommand{\CCGdLS}{\HepChemical{C}{17.072}{}\xspace}
\newcommand{\CCLAB}{\HepChemical{C}{17.14}{}\xspace}
\newcommand{\CCtf}{\HepChemical{C}{24}{}\xspace}
\newcommand{\CCN}{\HepChemical{C}{n}{}\xspace}
\newcommand{\COGdLS}{\HepChemical{O}{0.0126}{}\xspace}
\newcommand{\CNGdLS}{\HepChemical{N}{0.0037}{}\xspace}
\newcommand{\CGdGdLS}{\HepChemical{Gd}{0.0015}{}\xspace}
\newcommand{\CClT}{\HepChemical{Cl}{3}{}\xspace}
\newcommand{\CCrt}{\HepChemical{Cr}{2}{}\xspace}
\newcommand{\COT}{\HepChemical{O}{3}{}\xspace}
\newcommand{\CAlt}{\HepChemical{Al}{2}{}\xspace}
%
% Chemicals - Compounds
%
\newcommand{\CCsHF}{\CCs\kern-0.2em\CHFi}
\newcommand{\CCnHot}{\CCn\kern-0.2em\CHot}
\newcommand{\CCH}{CH\xspace}
\newcommand{\CCNHtN}{\CCN\kern-0.2em\CHtN}
\newcommand{\CCHLAB}{\CCLAB\kern-0.2em\CHLAB}
\newcommand{\CHtO}{\CHt{O}\xspace}
\newcommand{\CGdClT}{Gd\CClT\xspace}
\newcommand{\CHF}{HF\xspace}
\newcommand{\CHCl}{HCl\xspace}
\newcommand{\CCrtOT}{\CCrt\kern-0.25em\COT}
\newcommand{\CHNOT}{HN\COT}
\newcommand{\CAltOT}{\CAlt\kern-0.25em\COT}
\newcommand{\CBaTiOT}{BaTi\kern0.05em\COT}
\newcommand{\CNaI}{NaI\xspace}
\newcommand{\CCHt}{\HepChemical{C}{}{}\CHt}
\newcommand{\CCHT}{\HepChemical{C}{}{}\CHT}
\newcommand{\CCHf}{\HepChemical{C}{}{}\CHf}
\newcommand{\CTMHA}{\CCn\kern-0.2em\CHoe\kern-0.2em\COt}
\newcommand{\CTMHAm}{\CCn\kern-0.2em\CHoS\kern-0.2em\COt}
\newcommand{\CTMHAM}{\CCn\kern-0.2em\CHoS\kern-0.2em\COtM}
\newcommand{\CPPO}{\CCoF\kern-0.2em\CHoo NO}
\newcommand{\CbisMSB}{\CCtf\kern-0.2em\CHtt}
\newcommand{\CGdLS}{\CCGdLS\kern-0.2em\CHGdLS\kern-0.2em\COGdLS\kern-0.2em\CNGdLS\kern-0.2em\CGdGdLS}
%
% Table-related
%
\colorlet{mrocol}{ProcessBlue!100!}
\colorlet{lrocol}{SkyBlue!50!}
\newcommand{\sfbL}{\sffamily\bfseries\Large}
\newcommand{\sfbl}{\sffamily\bfseries\large}
\newcommand{\sfs}{\sffamily\small}
\newcommand{\rmbL}{\rmfamily\bfseries\Large}
\newcommand{\rmbl}{\rmfamily\bfseries\large}
\newcommand{\rms}{\rmfamily\small}
\newcommand{\Tstrut}{\rule{0pt}{2.4ex}}
\newcommand{\Bstrut}{\rule{1ex}{0pt}}
\newcommand{\numlb}[1]{\num[color=Tan]{#1}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}m{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
%\def\geantFour  {\mbox{\tt GEANT4}\xspace}
\def\geantFour  {\mbox{\scshape Geant4}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}
%
%  From Accelerator
%
\def\tenTo#1#2{\ensuremath{10^{#1#2} \cms}\xspace}
\newcommand{\EE}[1] {\ensuremath{\times 10^{#1}}\xspace}
\newcommand{\EEb}[1] {\ensuremath{\times \mathbf{10}^{\mathbf{#1}}}\xspace}
\newcommand{\PM}[2] {\ensuremath{^{+#1}_{-#2}}\xspace}

% Spin Polarization common symbols
\def\ze#1   {\ensuremath{\zeta_{#1}}\xspace}
\newcommand{\VE}[1]  {\ensuremath{\vec{\mathrm{#1}}}\xspace}

% Electrical units
\def\amp    {\ensuremath{{\rm \,\mathrm{A}}}\xspace}
\def\mA     {\ensuremath{{\rm \,\mathrm{mA}}}\xspace}
\def\muA     {\ensuremath{\mu\mathrm{A}}\xspace}
\def\kA	    {\ensuremath{{\,\mathrm{kA}}}\xspace}
\def\nC     {\ensuremath{{\,\mathrm{nC}}}\xspace}
\def\pC     {\ensuremath{{\,\mathrm{pC}}}\xspace}
\def\Ohm    {\ensuremath{{\,\Omega}}\xspace}
\def\mOhm   {\ensuremath{{\,\mathrm{m}\Omega}}\xspace}
\def\kOhm   {\ensuremath{{\,\mathrm{k}\Omega}}\xspace}
\def\MOhm   {\ensuremath{{\,\mathrm{M}\Omega}}\xspace}
\def\V     {\ensuremath{{\,\mathrm{V}}}\xspace}
\def\kV     {\ensuremath{{\,\mathrm{kV}}}\xspace}
\def\MV     {\ensuremath{{\,\mathrm{MV}}}\xspace}
\def\mV     {\ensuremath{{\,\mathrm{mV}}}\xspace}	
\def\Tesla  {\ensuremath{{\,\mathrm{T}}}\xspace}
\def\Gauss  {\ensuremath{{\,\mathrm{G}}}\xspace}
\def\kGauss  {\ensuremath{{\,\mathrm{kG}}}\xspace}
\def\dB     {\ensuremath{{\,\mathrm{dB}}}\xspace}
\def\Henry  {\ensuremath{{\,\mathrm{H}}}\xspace}

% SI energy unit
\def\J      {\ensuremath{{\,\mathrm{J}}}\xspace}
\def\kJ     {\ensuremath{{\,\mathrm{kJ}}}\xspace}
\def\MJ     {\ensuremath{{\,\mathrm{MJ}}}\xspace}

\def\Jpgm   {\ensuremath{{\,\mathrm{J/g}}}\xspace}

% Power
\def\Watt      {\ensuremath{{\,\mathrm{W}}}\xspace}
\def\MW     {\ensuremath{{\,\mathrm{MW}}}\xspace}
\def\kW     {\ensuremath{{\,\mathrm{kW}}}\xspace}


% Frequency
\def\Hz     {\ensuremath{{\rm \,Hz}}\xspace}
\def\MHz    {\ensuremath{{\rm \,MHz}}\xspace}
\def\GHz    {\ensuremath{{\rm \,GHz}}\xspace}
\def\kHz    {\ensuremath{{\rm \,kHz}}\xspace}

% Flux
\def\Hzpmma {\ensuremath{{\rm \,Hz/mm^2}}\xspace}
\def\kHzpmma {\ensuremath{{\rm \,kHz/mm^2}}\xspace}

\def\Hzpcma {\ensuremath{{\rm \,Hz/cm^2}}\xspace}
\def\kHzpcma {\ensuremath{{\rm \,kHz/cm^2}}\xspace}

% Neutron fluence, flux
\def\neqpcma {\ensuremath{{\,{\rm n}_{eq}/{\rm cm^2}}}\xspace}
\def\neqpcmaps  {\ensuremath{{\,{\rm n}_{eq}/{\rm cm^2/s}}}\xspace}
\def\neqpcmapyr  {\ensuremath{{\,{\rm n}_{eq}/{\rm cm^2/yr}}}\xspace}



% Time
\def\msec   {\ensuremath{{\rm \,ms}}\xspace}
\def\nsec   {\ensuremath{{\rm \,ns}}\xspace}

% Pressure
\def\Torr  {\ensuremath{{\rm \,Torr}}\xspace}
\def\nTorr  {\ensuremath{{\rm \,nTorr}}\xspace}
\def\Pa     {\ensuremath{{\rm \,Pa}}\xspace}
\def\MPa    {\ensuremath{{\rm \,MPa}}\xspace}

% Length
\def\picom  {\ensuremath{{\rm \,pm}}\xspace}
\def\km  {\ensuremath{{\rm \,km}}\xspace}

% Area
%(in babarsym) \def\mbarn  {\ensuremath{{\rm \,mbarn}}\xspace}

% Angle
\def\muRad  {\ensuremath{{\, \mu \rm rad}}\xspace}

% Force
\def\N     {\ensuremath{{\rm \,N}}\xspace}
\def\kN    {\ensuremath{{\rm \,kN}}\xspace} 
\def\kNpmm {\ensuremath{{\rm \,kN/mm}}\xspace}


\def\bets  {\ensuremath{{\beta^{\star}}}\xspace}
\def\betxs  {\ensuremath{{\beta_{x}^{\star}}}\xspace}
\def\betys  {\ensuremath{{\beta_{y}^{\star}}}\xspace}

\def\betx   {\ensuremath{{\beta_{x}}}\xspace}
\def\bety   {\ensuremath{{\beta_{y}}}\xspace}


\def\epsx   {\ensuremath{{\varepsilon_{x}}}\xspace}
\def\epsy   {\ensuremath{{\varepsilon_{y}}}\xspace}

\def\xix  {\ensuremath{{\xi_{x}}}\xspace}
\def\xiy  {\ensuremath{{\xi_{y}}}\xspace}

\def\thx  {\ensuremath{{\theta}}\xspace}
\def\piwi {\ensuremath{{\varphi}}\xspace}
\def\CW   {CW\xspace}
\def\br   {\ensuremath{B\rho}\xspace}
\def\thr  {\ensuremath{\theta_{r}}\xspace}

% Note: original symbol Bz conflicts with what is defined in babarsym
\def\Bzed   {\ensuremath{B_{z}}\xspace}

\def\Be   {Be\xspace}
\def\Cu   {Cu\xspace}
\def\Au   {Au\xspace}
\def\CO2  {$\mathrm{CO}_2$\xspace}


\newcommand{\TODO}[1] {{\color{red} \mbox{ #1}}\xspace}


% Note: for Debbie Ceder, 10/8/2015
%\newcommand{\gtwid}{\mathrel{\raise.3ex\hbox{$>$\kern-.75em\lower1ex\hbox{$\sim$}}}}
%\newcommand{\ltwid}{\mathrel{\raise.3ex\hbox{$<$\kern-.75em\lower1ex\hbox{$\sim$}}}}


==> LZPaperSupport/commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% SuperB Detector Technical Design Report
% User defined commands and symbols
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Define symbols
\input{LZsym}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define command to begin new section/subsection/subsubsection, so that it's easy to change it
% Use:
% \tdrchap for the chapter/subsystem level
%  \tdrsec for the section level
%     \tdrsubsec
%        \tdrsubsubsec
%           \tdrparagraph
%
% Command to include chapters. Convention is that the main file name is the same as the chapter directory
% For example : SVT/SVT.tex
% This requires the 'import' package that takes care of handling the subdirectories
% \subimport* means include from subdir without looking in TEXINPUTS
% Used in conjuction of the \tdrchap command, it automatically defines a chapter
% label, in the form of chap:dirname, such as \label{chap:SVT} 
%
\newcommand{\ChapLabel}{chap:empty}
\newcommand{\BibLabel}{empty:bib}
\newcommand{\SecPre}{empty}
\newcommand{\FloatPre}{empty}
\newcommand{\tdrinclude}[1]
{
%\befchap
\renewcommand{\ChapLabel}{chap:#1} % define the label for the chapter
\renewcommand{\BibLabel}{#1S:bib} % define the label for the chapter
\renewcommand{\SecPre}{#1}
\renewcommand{\FloatPre}{#1}
\subincludefrom{#1/}{#1}
\wlog{In tdrinclude command}
\wlog{\ChapLabel}
%\aftchap
}

\newcommand{\tdrchap}[2][\ChapLabel]
{
   \ifx#1\ChapLabel
     \chapter{#2\ifKL\space\texttt{#1}\fi}
     \label{#1}
   \else
    \renewcommand{\ChapLabel}{chap:#1} % define the label for the chapter
    \renewcommand{\BibLabel}{#1S:bib} % define the label for the chapter
    \renewcommand{\SecPre}{#1}
    \renewcommand{\FloatPre}{#1}
    \chapter{#2\ifKL\space\texttt{\ChapLabel}\fi}
    \label{\ChapLabel}
   \fi
}

\newcommand{\tdrsec}[2][\Alph{section}]
{
   \section{#2\ifKL\space\texttt{\SecPre S:#1}\fi}
   \label{\SecPre S:#1}
}

\newcommand{\tdrsubsec}[2][\Alph{section}\alph{subsection}]
{
   \subsection{#2\ifKL\space\texttt{\SecPre Ss:#1}\fi}
   \label{\SecPre Ss:#1}
}

\newcommand{\tdrsubsubsec}[2][\Alph{section}\alph{subsection}\Roman{subsubsection}]
{
   \subsubsection{#2\ifKL\space\texttt{\SecPre Sss:#1}\fi}
   \label{\SecPre Sss:#1}   
}

\newcommand{\tdrparagraph}[2][\Alph{section}\alph{subsection}\Roman{subsubsection}\roman{paragraph}]
{
   \paragraph{#2\ifKL\space\texttt{\SecPre Sssp:#1}\fi}
   \label{\SecPre Sssp:#1}
}

\renewcommand{\bibsection}{\tdrsec[bib]{Bibliography}}

\newcommand{\tdrtcaption}[3][\arabic{section}.\arabic{subsection}.\arabic{table}]
{
   \caption[#2\ifKL\space\texttt{\FloatPre t:#1}\fi]{#3\ifKL\space\texttt{\FloatPre t:#1}\fi}
   \label{\FloatPre t:#1}
}

\newcommand{\tdrfcaption}[3][\arabic{section}.\arabic{subsection}.\arabic{figure}]
{
   \caption[#2\ifKL\space\texttt{\FloatPre f:#1}\fi]{#3\ifKL\space\texttt{\FloatPre f:#1}\fi}
   \label{\FloatPre f:#1}
}

%\iftrue
%\titleformat{\section}%
%  {\raggedsection\normalfont\sectfont\Large\bfseries}%{\thesection}%
%  {0.4em}%
%  {\phantomsection}%
%  [\vspace{0.5ex}\centerline{\rule[0.15in]{0.9\columnwidth}{2pt}}\vspace*{-1.5ex}]
%\fi

%%%
% Define the detpth for numbering sections and including them in TOC
%
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}

%
% commands handling new page at the end of chapters
%
\newcommand{\befchap}{\relax}
\newcommand{\aftchap}{\relax}
%

\long\def\ignore#1{\relax}
\let\BaBar=\babar

%%--- define \url font to be small normal font
%\makeatletter
%\def\url@tdrstyle{%
%  \@ifundefined{selectfont}{\def\UrlFont{\normalfont}}{\def\UrlFont{\normalfont\smaller}}}
%\makeatother
%\urlstyle{tdr}
%%\urlstyle{same}

%%--- put bibliography in a section for scrbook
\makeatletter
\renewcommand*\bib@heading{%
  \section{\bibname}
  \@mkboth{\bibname}{\bibname}
}
\makeatother

%%
%% floats
%%

\renewcommand{\topfraction}{.85} % max fraction of floats at top
\renewcommand{\bottomfraction}{.70} % max fraction of floats at bottom
\renewcommand{\textfraction}{.15}
\renewcommand{\floatpagefraction}{.66} % float-only pages
\renewcommand{\dbltopfraction}{.66}
\renewcommand{\dblfloatpagefraction}{.66} % float-only pages

%%--- max number of floats in text pages
\setcounter{topnumber}{9}
\setcounter{bottomnumber}{9}
\setcounter{totalnumber}{20}
\setcounter{dbltopnumber}{9}

\iffalse
\setlength\floatsep{1.25\baselineskip plus 3pt minus 2pt}
\setlength\textfloatsep{1.25\baselineskip plus 3pt minus 2pt}
\setlength\intextsep{1.25\baselineskip plus 3pt minus 2 pt}
\fi

%% bold math in section titles
\makeatletter
\DeclareRobustCommand\bfseries{%
  \not@math@alphabet\bfseries\mathbf
  \fontseries\bfdefault\selectfont\boldmath}
\DeclareRobustCommand*{\bm}[1]{%
    \mathchoice{\bmbox{\displaystyle}{#1}}%
               {\bmbox{\textstyle}{#1}}%
               {\bmbox{\scriptstyle}{#1}}%
               {\bmbox{\scriptscriptstyle}{#1}}}
\DeclareRobustCommand*{\bmbox}[2]{\mbox{\bfseries$#1 #2$}}
\makeatother

\setcapindent{0pt} % to eliminate hanging indent from figure captions

% captions in sans serif
\setkomafont{captionlabel}{\normalfont\sffamily\bfseries}
\setkomafont{caption}{\normalfont\sffamily}
\setkomafont{pagefoot}{\normalfont\sffamily}
\setkomafont{pagenumber}{\normalfont\sffamily}
\setkomafont{pagehead}{\normalfont\sffamily}

%
% longtable caption default
%
\newcommand{\ltbcp}{lngtab}

%
% Modified todo command
%
\newcounter{lzcomm}
\newcommand{\lzcomm}[3][]{%
 % options, initials, comment
 \refstepcounter{lzcomm}%
 { \todo[#1]{%
   \textbf{\uppercase{#2}\thelzcomm:}~#3}}}


%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

